Inv-ASKIT: A Parallel Fast Diret Solver for Kernel Matrices

We present a parallel algorithm for computing the approximate factorization of an $N$-by-$N$ kernel matrix. Once this factorization has been constructed (with $N \log^2 N $ work), we can solve linear systems with this matrix with $N \log N $ work. Kernel matrices represent pairwise interactions of points in metric spaces. They appear in machine learning, approximation theory, and computational physics. Kernel matrices are typically dense (matrix multiplication scales quadratically with $N$) and ill-conditioned (solves can require 100s of Krylov iterations). Thus, fast algorithms for matrix multiplication and factorization are critical for scalability. Recently we introduced ASKIT, a new method for approximating a kernel matrix that resembles N-body methods. Here we introduce INV-ASKIT, a factorization scheme based on ASKIT. We describe the new method, derive complexity estimates, and conduct an empirical study of its accuracy and scalability. We report results on real-world datasets including "COVTYPE" ($0.5$M points in 54 dimensions), "SUSY" ($4.5$M points in 8 dimensions) and "MNIST" (2M points in 784 dimensions) using shared and distributed memory parallelism. In our largest run we approximately factorize a dense matrix of size 32M $\times$ 32M (generated from points in 64 dimensions) on 4,096 Sandy-Bridge cores. To our knowledge these results improve the state of the art by several orders of magnitude.

==> hier.tex <==
Fast kernel summations or solvers based on treecodes
exploit the hierarchical low-rank structure of $K$ with a 
nested spatial partitioning.
Quad-tree and oct-tree are often used in $d=2,3$, and KD-tree is used
in high $d$ to reduce the cost spent on building the tree.
For different treecodes and representations, we refer the reader
to \cite{ambikasaran2013fast}, which classifies these matrices according 
to their admissibility, nested low-rank structure and the way 
their low-rank structures can be constructed.
In \tabref{tab:contrast},
we summarize three different types of matrices: FMM, 
HSS and HODLR matrices, and we introduce a more robust representation ASKIT.

\begin{table}[!htp]
\centering
{%\footnotesize
  \begin{tabular}{lcrrr}
  \hline
  Method       && Admissibility
                & Solver 
                & Factorization \\
  \cline{1-1} \cline{3-5} 
  FMM   && neighbor & $\MA{O}(N)$ & $\MA{O}(N)$  \\
  HSS   &&  sibling & $\MA{O}(N)$ & $\MA{O}(N)$--$\MA{O}(N^{2})$ \\
  HODLR &&  sibling & $\MA{O}(N\log{N})$ & $\MA{O}(N\log^{2}{N})$ \\
  \hline
  \end{tabular}
}
  \caption{Comparison between different methods. }
  \label{tab:contrast}
\end{table}

HSS matrices are subsets of HODLR matrices, and both matrices have weak admissibility,
which means that the off-diagonals of $K$ are low-rank.
Constructing the low-rank structure for both matrices can either be analytically
(1st order function approximation)
or algebraically (rank-revealing factorization), 
but HSS can achieve a lower constructing complexity
with an analytic construction due to the nested low-rank assumption. 
With $ULV$ decomposition, HSS matrices can be
solved in $\MA{O}(N)$ \cite{chandrasekaran2006fast}. 
On the other hand, HODLR metrices take $\MA{O}(N\log{N})$
\cite{ambikasaran2013mathcal} by
the Sherman-Morrison-Woodbury formula. Different from HSS and HODLR, 
FMM matrices use a regular spatial tree instead of KD-tree, since the strong admissibility 
requires the exact neighbor list to control the accuracy. 
The construction must be analytic to reach $\MA{O}(N)$ \cite{ambikasaran2014inverse}, 
and it's solved by expanding the dense kernel matrix into a pattern symmetric sparse matrix.

Despite that these matrices can be solved fast with controllable accuracy,
yet only a limited subset of $K$ is qualified.
We take a $10D$ Gaussian kernel matrix as an example.
FMM ends up with exponential work, since the regular tree partitioning results 
in $2^{10}$ children in each level. 
The off-diagonal of $K$ is almost full-rank; thus, HSS and HODLR matrices end up 
having cubical works, which are no longer fast anymore.
%Given the desired accuracy, the complexity usually scales badly in high $d$
%or when the kernel function lost its smoothness.
%For example, HSS and HODLR may take $\MA{O}(N^3)$ to solve a $10D$ Gaussian
%kernel matrix with a desired accuracy, which is no longer fast anymore.

%(Interestingly, it takes $\MA{O}(N^2)$ to
%compress algebraically if using raw data. There must be some methods to lead
%to $\MA{O}(N)$ compression.)

%{\bf HSS:} Here we demonstrate the algebraic compression steps of a 2-level
%HSS matrix. In the upward level-1 compression, 
%$K_{\alpha_2 \times \alpha_7 \setminus \alpha_2} 
%\sim U_{1}W_{\alpha_2 \times \alpha_7 \setminus \alpha_2}$ is done by some
%pivoting QR factorization, and similarly
%$K_{\alpha_1 \times \alpha_7 \setminus \alpha_1} 
%\sim U_{2}F_{\alpha_1 \times \alpha_7 \setminus \alpha_1}$.
%In level-2,
%\begin{equation}
%  K_{\alpha_3 \times \alpha_7 \setminus \alpha_3} \sim 
%  \begin{bmatrix}
%    U_{1}F_{\alpha_1 \times \alpha_7 \setminus \alpha_1} \\
%    U_{2}F_{\alpha_2 \times \alpha_7 \setminus \alpha_2}
%  \end{bmatrix}
%  =
%  \begin{bmatrix}
%    U_{1}R_{1} \\
%    U_{2}R_{2}
%  \end{bmatrix}
%  F_{\alpha_3 \times \alpha_7 \setminus \alpha_3}  
%\end{equation}
%In the downward level-1 compression, LR factorization (the transpose version of QR)
%can factor $F_{\alpha_3 \times \alpha_4} = B_4V^{H}_5$, and similarly 
%$F_{\alpha_4 \times \alpha_3} = B_5V^{H}_4$.
%In level-2,
%\begin{equation}
%  \begin{bmatrix}
%    W_{4} \\
%    W_{5}
%  \end{bmatrix}
%  =
%  \begin{bmatrix}
%    V_{4}^{H} \\
%    V_{5}^{G}
%  \end{bmatrix}
%  F_{\alpha_3 \times \alpha_7 \setminus \alpha_3}
%\end{equation}
%And finally, $W_{4} = W_{4}$  


%Unfortunately, even that HSS and HODLR have the most relaxed assumptions, 
%but still not all kernel matrices in an arbitrary $d$ dimensional space 
%can be accurately represented in these formats.
%HSS and HODLR are usually built with KD-tree, which recursively subdivides
%the space into clusters. The binary tree partition is one of the best known
%scheme to partition data points in a high dimensional space, which avoids
%growning clusters exponentially in the typycal 2D quad-tree and 3D oct-tree
%partitioning.
%The drawback of the KD-tree partitioning is that the neighbor can hardly be
%define in the KD-tree; thus, the near-far interaction 
%Compressing the off-diagonals results in lose of accuracy. 



%To compute the summation or the inverse fast, interactions between clusters
%are classified into near and far interactions.  
%In low $d$, the near-far interaction list is decided by the admissibility,
%which is strictly defined using the neighbor relation between clusters. 
%However, in higher $d$ this approach ends up having exponential complexity.  
%Neighbors in a binary tree partition are difficult to define, and it's
%likely that all other clusters are neighbors in high $d$.
%Abandoning the neighbor relation, an nearest-neighbor pruning is adopted 
%by ASKIT, which gives birth to the idea of a robust hierarchical 
%off-diagonal low rank matrix. 
%In this robust representation, we assume that $K$ consists a sparse matrix
%and a HSS or a HODLR matrix.
%The HSS or the HODLR matrix represents the self and the far interaction,
%and the sparse matrix represents the near interaction. 
% In the case of HSS matrix, the factorization is expressed as:
%\begin{equation}
%  K^{-1} = (A + USV)^{-1}
%  \label{e:sparseandlowrank}
%\end{equation}
    
{\bf Robust hierarchical representation:}
%When the off-diagonals of the $K$ is full-rank, HSS and HODLR matrices end up 
%having $\MA{O}(N^3)$ complexity. 
With this observation,
a more robust representation is required to maintain the accuracy without 
increasing the complexity too much. 
One hope is that the full-rank off-diagonal block can be 
decomposed into a low-rank matrix and a sparse full-rank matrix. 
This decomposition is called RPCA (Robust Principle Component Analysis)
\cite{candes2011robust,wright2009robust}, originally studied to recover
corrupted low-rank matrices.
By splitting the sparse matrix $E$ from $K$, the low-rank and the diagonal parts
$H$ can be efficiently represented as a HODLR matrix. 
We denote this robust representation as ASKIT when the pattern of $E$ is decided
by the $\kappa$ nearest-neighbor of $\XX$.
%The formal definition of the RPCA of a kernel matrix $K$ is to find a low-rank $A$ 
%and sparse $E$ with a restricted convex optimization problem. 
%\begin{equation}
%\label{e:rpca}
%  \min_{A,E}\|A\|_{*}+\gamma\|E\|_{1}, s.t. \|K-A-E\|_{2} \leq \epsilon.
%\end{equation}

\textbf{Treecode:}
If $K$ is symmetric, a nested binary partitioning of $K$ can be efficiently
stored as a complete binary tree. Each node $\alpha$ contains a subset of 
$\XX$ stored by their indices. To repartition $\alpha$, we use notation
$l(\alpha)$ and $r(\alpha)$ to denote the left and right children where
$\alpha = l(\alpha) \cup r(\alpha)$ and
$l(\alpha) \cap r(\alpha) = \phi$.
In the matrix represenation, the diagonals of $K$ are further partitioned 
into 2-by-2 matrices shown in \eqref{e:partitioning} in each level.
Thus, at level-$l$, there are $2^{l}$ diagonal blocks $K^{(l)}_{11}$ to
$K^{(l)}_{2^{l}2^{l}}$.
\begin{equation}
  \label{e:partitioning}
  K^{(0)} = 
  \begin{bmatrix}
  K_{11}^{(1)} & K_{12}^{(1)} \\
  K_{21}^{(1)} & K_{22}^{(1)} \\
  \end{bmatrix}
  =
  \begin{bmatrix}
  K_{11}^{(2)} & K_{12}^{(2)} & \multicolumn{2}{c}{\multirow{2}{*}{$K_{12}^{(1)}$}} \\
  K_{21}^{(2)} & K_{22}^{(2)} & \multicolumn{2}{c}{} \\
  \multicolumn{2}{c}{\multirow{2}{*}{$K_{21}^{(1)}$}} & K_{33}^{(2)} & K_{34}^{(2)} \\
  \multicolumn{2}{c}{} & K_{43}^{(2)} & K_{44}^{(2)} \\
  \end{bmatrix}       
\end{equation}
In each level, the off-diagonal block is approximate by a rank-$s$ decomposition ($UV$) 
and a sparse matrix ($E$) shown in \eqref{e:askit}. The sparse matrix $E$ is
split out recursively from $K$, and the remaining part is a HODLR matrix $H$.
\begin{equation}
  \label{e:askit}
  H + E = 
  \begin{bmatrix}
  K_{11}^{(1)} & U_{1}^{(1)}V_{2}^{(1)} \\
  U_{2}^{(1)}V_{1}^{(1)} & K_{22}^{(1)} \\
  \end{bmatrix} 
  +
  \begin{bmatrix}
  & E_{12}^{(1)} \\
  E_{21}^{(1)} & \\
  \end{bmatrix} 
\end{equation}
%By spliting out the sparse matrix $E$ at each level, the remaining part $H^{(0)}$ is
%a HODLR matrix. 
By factorizing $H$ in to \eqref{e:hodlr}, 
we observe that the diagonal blocks can be factorized recursively,
and $I + \tilde{U}^{(1)}V^{(1)}$ can be inverted fast 
by the Shermon-Morrison-Woodbury formula \eqref{e:smw}. 
\begin{equation}
\label{e:hodlr}
  H = 
  \begin{bmatrix}
  K_{11}^{(1)} &  \\
   & K_{22}^{(1)} \\
  \end{bmatrix}
  (
  I
  +
  \begin{bmatrix}
  \tilde{U}_{1}^{(1)} &  \\
  & \tilde{U}_{2}^{(1)} \\
  \end{bmatrix}
  \begin{bmatrix}
  & V_{2}^{(1)} \\
  V_{1}^{(1)} & \\
  \end{bmatrix}
  ).
\end{equation}
Here
$\tilde{U}_{1}^{(1)} = (K_{11}^{(1)})^{-1}U_{1}^{(1)}$ 
and $\tilde{U}_{2}^{(1)} = (K_{22}^{(1)})^{-1}U_{2}^{(1)}$.
In the leaf level, diagonals $K_{11}^{(1)}$ and $K_{22}^{(1)}$ are inverted by
LU factorization or SVD (Singular Value Decomposition).
Otherwise, $K_{11}^{(1)}$ and $K_{22}^{(1)}$ are inverted recursively by
\eqref{e:partitioning} and \eqref{e:askit}.
\begin{equation}
\label{e:blocksmw}
  (I + \tilde{U}^{(1)}V^{(1)})^{-1} = I - 
  %\begin{bmatrix}
  %\tilde{U}_{1}^{(1)} &  \\
  %& \tilde{U}_{2}^{(1)} \\
  %\end{bmatrix}
  \tilde{U}^{(1)}
  \begin{bmatrix}
  I & V_{2}^{(1)}\tilde{U}_{2}^{(1)} \\ 
  V_{1}^{(1)}\tilde{U}_{1}^{(1)} & I \\
  \end{bmatrix}^{-1}
  \tilde{V}^{(1)}
  %\begin{bmatrix}
  %& V_{2}^{(1)} \\
  %V_{1}^{(1)} & \\
  %\end{bmatrix}
\end{equation}
In \eqref{e:smw}, the Shermon-Morrison-Woodbury formula reduces the 
linear system to a $2s$-by-$2s$ linear system, which is again factorized 
by LU factorization or SVD. 
%Together, if we assume that $s$ in constant to $N$ in the magnitude, then 
%factorizing \eqref{e:hodlr} recursively takes 
%$\MA{O}(N\log^2{N})$, and solving \eqref{e:hodlr} using \eqref{e:smw} 
%recursively takes $\MA{O}(N\log(N))$.

{\bf Low rank approximation and RPCA:}
%In the robust representation, each off-diagonal block is decomposed
%into a rank-$s$ update $UV$ and a sparse matrix $E$.
The RPCA problem is typically solved in the form of \eqref{e:rpca} as a convex 
optimization problem.
In the following, we only take $K_{12}$ as an example, but $K_{21}$ can be 
decomposed in the same way.
%Despite that $U_{1}$, $V_{2}$ and $E_{12}$ are all unknown, 
\begin{eqnarray}
\label{e:rpca}
  \min_{U_1,V_2,E_{12}}\|U_1V_2\|_{*}+\gamma\|E_{12}\|_{1}, \\
  s.t. \|K_{12}-U_1V_2-E_{12}\|_{2} \leq \epsilon.
\end{eqnarray}
Here $\|\|_{*}$ is the nuclear norm, $\gamma$ is the weight constant used to describe preference between
the sparsity of $E_{12}$ and the rank of $U_1V2$, and $\epsilon$ is the desired accuracy.
\eqref{e:rpca} is solved with the help of argument Largange multiplier,
and gradient descent methods are typically used to find the minimum 
iteratively.
In each iteration $E_{12}$ will be updated by $K_{12}-U_1V_2$ with a value threshold, 
and $U_1V_2$ is updated by a full SVD or Lanczos SVD depending on the current 
rank and the problem size. 
This results in $\MA{O}(N^{3})$, which is not practical when 
we try to develop a $\MA{O}(N\log^{2}{N})$ solver.
Alternatively with the geometric insight, ASKIT assume the structure of 
$E_{12}$ is related to the
nearest-neighbor distribution. By removing those nearest-neighbors 
elements, $K_{12}-E_{12}$ becomes numerical low-rank, and $U_1V_2$ 
can be approximate 
by interpolation decomposition (ID) \cite{cheng2005compression}.


{\bf Interpolation decomposition:}
ASKIT uses a nested ID with an important sampling to reduce the complexity.
Given $G = K_{12} = K(\alpha,\beta)$ represents the interaction
between two siblings $\alpha$ and $\beta$,
ID is a rank-$s$ decomposition such that 
$G \simeq G_{col}P$ where $G_{col}$ contains $s$ columns of $G$.
These columns are stored by their indices in $\SK_{\beta} \subseteq
\beta$, and we call the points with these indices skeletons of $\beta$.

In ASKIT, column-pivoting QR factorization suggested 
by Businger and Golub \cite{businger1965linear} is employed to find 
these skeleton columns.
For example, let $\alpha$ and $\beta$ are leaf nodes, then 
\eqref{e:leafid} shows that $U$ is generated from those
skeleton columns $K(\alpha,\SK_{\beta})$, and $V$ is the projection matrix $P$.
$\SK_{\beta}$ are the first $s$ pivoting columns of $K(\alpha,\beta)$ in the
QR factorization (\texttt{GEQP3}), and
$P=K(\alpha,\SK_{\beta})^{\dagger}K_{12}^{(2)}$
is solved by the pseudo-inverse (\texttt{GELS}).
\begin{equation}
\label{e:leafid}
  K_{12}^{(2)} = K(\alpha,\SK_{\beta})P 
  = U_{1}^{(2)}V_{2}^{(2)}
\end{equation}
To prevent $K(\alpha,\beta)$ from growing too larger, 
the non-leaf node skeletons are selected from the union
of the children skeletons to reduce the complexity.
i.e. $G = K(\alpha,\SK_{l(\beta)} \cap \SK_{r(\beta)})$.
\eqref{e:innerid} shows that when $\alpha$ and $\beta$ are non-leaf
nodes, $\SK_{\beta}$ are the pivoting columns of 
$K(\alpha, \SK_{l(\beta)} \cap \SK_{r(\beta)})$, and
$P=K(\alpha,\SK_{\beta})^{\dagger}K_{12}^{(2)} =
K(\alpha,\SK_{\beta})^{\dagger}K(\alpha,\SK_{l(\beta)}\cap\SK_{r(\beta)})$
only contains $2s$ skeleton columns from it's children.
To recover $V$, we reconstruct from its children and $P$ using:
\begin{equation}
\label{e:innerid}
  K_{12}^{(1)} = K(\alpha,\SK_{\beta})P
  \begin{bmatrix}
  V_{3}^{(2)} &   \\
        & V_{4}^{(2)}\\
  \end{bmatrix}
  = U_{1}^{(1)}V_{2}^{(1)}.
\end{equation}
%We show the rank-$s$ ID of $K_{12}$ in \eqref{e:id} where
%$U_{1}$ can be evaluated as $K(l(\alpha),\SK_{r(\alpha)})$, and 
%$V_{2} = \Ker(l(\alpha),\SK_{r(\alpha)})^{\dagger}K_{12}$ is solved as
%a least-square problem.
%to minimize
%low-rank representation. 
%Column-pivoting QR factorization is
%emploied to find these skeleton columns, and $V$ is solved as a least-square
%problem such that $\|K-K(:,\SK)V\|$ is small.

Given that $G$ has $m$ columns, ID has a looser error bound \eqref{e:skeletonerror}
than SVD.
Let $\sigma_{s+1}(G)$ be the $(s+1)$th singular value of $G$,
the error of ID grows with $m$,  
but the complexity can be linear to the problem size if
the nested skeletonization is used in non-leaf nodes.
\begin{equation}
\label{e:skeletonerror}
  \|G-G_{col}P\|_2 \leq \sqrt{1+m(m-s)}\sigma_{s+1}(G)
\end{equation} 
To further reduce the complexity, an important sampling scheme can be used
to select pivoting rows. Important sampling in \ASKIT{} select rows from
the nearest-neighbors. This scheme is shown having a smaller error bound
than uniform sampling in \cite{march2015robust}.


%The weak adminisity assumption of HSS and HODLR 
%We further relax the HODLR matrix into its extended format, and we briefly 
%discuss how this extened format can be solved fast.
%In each level of the partitioning shown in \eqref{e:nearfar}, HODLR assumes 
%that diaagonal blocks $K_{11}$ and $K_{22}$ are full-rank, but the off-diagonals
%$K_{21}$ and $K_{12}$ can be approximate by some low-rank $UV$ factorization.
%This low-rank assumption is general not true, and $\|U_{1}V_{2}-K_{12}\|_2$ can
%be huge.
%To circonvent 
%Some interactions  data points in the sibling cluster is actually 
%
%While the HODLR matrix assume the off-diagonal can be approximate by some
%low-rank $UV$ factorization, the accuracy is lost due to the compression.
%Some interaction 
%
%However, the spirit of \eqref{e:globalshm} can be extended to the HODLR matrix, 
%which only requires a non-nested low rank structure. 
%Our goal is to express the kernel matrix $K$ in the following
%form:
%
%


==> par.tex <==
Given $p$ MPI processes and the distributed tree provided by \ASKIT{}, 
distributed \IASKIT{} is invoked from tree level-$\log{p}$ to the
root level. Without loss of generality, we assume $N$ and $p$ are powers 
of two, and each MPI process owns $n=N/p$ points corresponding to a 
subtree in level-$\log{p}$.
Each subtree is factorized and solved locally, but computing the tree nodes
above requires collaboration and communication.
We first illustrate the distributed algorithms, and later we analyze the
complexity. 

\textbf{Data Distribution.}
In \figref{fig:tree}, we show a 4-process distributed tree provided
by \ASKIT{}. In level-1, the root has two children $\alpha$ and $\beta$.
In level-$\log{4}$, $\alpha$ has two children $\lc(\alpha)$ and $\rc(\alpha)$
as well as $\beta$.
Each MPI process is labeled with different colors, and we label the
data they own including $\XX$, $\bu$, skeletons and projection matrices.
Processes in the same distributed tree node are grouped together
by the purple box to form a subcommunicator, and we use 
\{0, ..., $q-1$\} to denote the local MPI rank. 
In each non-root treenode, only \{0\} possesses the skeletons
and the projection matrix.

In each level, each MPI process only maintain a portion of 
$U$ and $V$ of the distributed node.
Thus, communication is required within and between each node in the 
same level during both factorization and solving phase.
\figref{fig:matrix} shows how $U$ and $V$ are distributed in the
tree we show in \figref{fig:tree}.
Each process is designed to own the $U$ (later overwritten by $W$) 
and $V$ portion with the same color, and the computation may require 
skeletons and the projection matrices from other processes.
Take the yellow process as an example.
In level-1, evaluating $V^{(1)}$ requires \{0\} (green) to broadcast the 
projection matrix $P_{\alpha[\tilde{\lc}\tilde{\rc}]}$. 
Evaluating $U^{(1)}$ requires skeletons $\tilde{\beta}$ from 
its sibling node (orange).
Factorizing $Z$ requires \{0\} to reduce all $VW$
parts in the same distributed node.
Solving \eqref{e:smw} requires both reducing $V\bu$ and broadcasting
$ZV\bu$ in the same node.  

\begin{figure}[!t]
  \centering
  \includegraphics[scale=.35]{figures/distributed_tree_v2.pdf}
  \caption{Distributed binary tree with 4 processes. The leafs of the 
  tree are the roots of each local tree.
  Each process possesses the data of its colored rectangle 
  region, and processes in the same treenode are group into
  a subcommunicator.}
  \label{fig:tree}
\end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[scale=.35]{figures/distributed_tree_v3.pdf}
  \caption{Distributed $U$ and $V$ factors. Each process
  only store the $U$ and $V$ portion of the same color in each
  level.}
  \label{fig:matrix}
\end{figure}

{\bf Factorization.}
In \algref{a:distributedfactor}, we present a recursive distributed 
factorization that traverses from level-$\log{p}$ to level-0.
In each level, \{0, ..., $\frac{q}{2}-1$\} will traverse the left child,
and \{$\frac{q}{2}$, ..., $q-1$\} will traverse the right child. 
We use \texttt{c} to denote the child node of $\alpha$.
Whether \texttt{c} is $\lc$ or $\rc$ depends on its local MPI rank.
%Similar to the local tree factorization, in each level \algref{a:distributedfactor}
%first splits out the sparse matrix $E$ by using $\kappa$-nearest neighbors.
%Then each node constructs its skeletons and
To satisfy the data dependency, \{0\} \texttt{Bcast} 
$P_{\tilde{\alpha}[\tilde{l}\tilde{r}]}$ to all processes in the node
and \texttt{Bcast} the skeleton $\tilde{\alpha}$ to all processes
in the sibling node.
Each process then computes the $U$ and $V$ portion it owns.
Once the $U$ portion is computed, \algref{a:distributedsolve} is called
to apply the inverse of $\tilde{K}^{-1}_{\alpha\alpha}$ to get $W$.
Finally, every process compute the its $VW$ portion, and 
\{0\} \texttt{Reduce} all $VW$ portion to factorize $Z$.


%In the level-$\log{p}$, 
%we first compute the $\SKa$ and $P$ using ID, and we can compute $V^{\log{\frac{p}{q}}}$ using
%\eqref{e:innerid}. Evaluating $U^{\log{\frac{p}{q}}}$ relies on the skeletons
%of its sibling, so we postpone the evaluation till reaching the parent level.
%For each non-leaf node, MPI processes in the same subcommunicator are subdivided into 
%left LC \{0, ..., $\frac{q}{2}-1$\} and right LC
%\{$\frac{q}{2}$, ..., $q-1$\}.
%\{0\} broadcasts $\SK_{l(\alpha)}$ to the right LC, 
%and \{$\frac{q}{2}$\} broadcasts $\SK_{r(\alpha)}$ to the left LC.
%With all skeletons, \{0\} can compute $\SKa$ and $P$ using ID and
%broadcasts $P$ to every processes in the LC.
%All processes can evaluate $U^{(\log{\frac{p}{q}}+1)}$ by using the skeletons just received
%and compute $V^{(\log{\frac{p}{q}})}$ by $P$ and $V^{(\log{\frac{p}{q}}+1)}$.
%Once $U^{(\log{\frac{p}{q}}+1)}$ has been evaluated, \algref{a:distributedsolve} 
%is called to solve $\tilde{U}^{(\log{\frac{p}{q}}+1)}$. 
%\{0\} reduces $V_{1}\tilde{U}_{1}$
%from the left LC and $V_{2}\tilde{U}_2$ from the right LC.
%Finally \eqref{e:smw} is factorized using LU factorization on \{0\}.
%Overall, the computation complexity $T_f(N,p)$ of
%\eqref{a:distributedfactor} is $\MA{O}(s^{2}\frac{N}{p}\log^{2}{p})$, and
%the communication complexity is $\MA{O}(s^{2}\log^3{p})$.



\begin{algorithm}[!htp]
\begin{algorithmic}
  \IF {$\alpha$ is at level-$\log{p}$}
    \STATE \texttt{Factorize($\alpha$)}.
  \ELSE
    \STATE \{$i<\frac{q}{2}$\} \texttt{DistributedFactorize}($\lc$, $\frac{q}{2}$).
    \STATE \{$i\geq\frac{q}{2}$\} \texttt{DistributedFactorize}($\rc$, $\frac{q}{2}$).
    \STATE \{0\} \texttt{Bcast} $P_{\tilde{\alpha}[\tilde{l}\tilde{r}]}$ inside the distributed node.
    \STATE \{$0\rightarrow\frac{q}{2}$\} \texttt{SendRecv} $\sk{\lc}$.
    \STATE \{0\} \texttt{Bcast} inside $\lc$ using the $\lc$ communicator.
    \STATE \{$\frac{q}{2}$\} \texttt{Bcast} inside $\rc$ using the $\rc$ communicator.
    \STATE \{$\frac{q}{2}\rightarrow0$\} \texttt{SendRecv} $\sk{\rc}$.
    \STATE Compute \eqref{e:innerid} to get the $U$ and $V$ portions.
    \STATE \{$i<\frac{q}{2}$\}$W=\texttt{DistributedSolve}(\lc, U, \frac{q}{2})$.
    \STATE \{$i\geq\frac{q}{2}$\}$W=\texttt{DistributedSolve}(\rc, U, \frac{q}{2})$.
    \STATE \{0, $\frac{q}{2}$\} \texttt{Reduce} $VW$.
    \STATE \{$\frac{q}{2}\rightarrow0$ \texttt{SendRecv} $VW$.
    \STATE \{0\} computes and LU factorizes $Z$.
  \ENDIF
\end{algorithmic}
\caption{{} \texttt{DistributedFactorize}($\alpha$,$q$)}
\label{a:distributedfactor}
\end{algorithm}


{\bf Solver.}
The distributed solver is also implemented using recursive bottom-up
traversal. \algref{a:solve} is called to solve the local tree while 
reaching level-$\log{p}$.
%We first compute the projection $V\bu$ on each process separatelu.
\{0\} reduces all portions of $V\bu$ and compute $ZV\bu$
where $Z$ was previously factorized in \algref{a:distributedfactor}.
%We solve \eqref{e:smw} to update $\tilde{V\bu}$, and we compute the backward
%projection and its update $\bu-\tilde{U}\tilde{V\bu}$. 
%Recall that each process owns its part of $V$ and $\bu$; thus, we 
%only need to reduce $V\bu$ to \{0\} for inversion. 
%The reduced $2s\times 2s$ system was previously factorized on \{0\},
%so it will reduce all $V\bu$ from everyone in the LC and solve \eqref{e:smw}.
$Z^{-1}V\bu$ is \texttt{Bcast} back to all processes by \{0\}, 
and each process updates its own$\bw$ 
by $\bu-WZ^{-1}V\bu$ to complete the solving phase.
%Overall, the computation complexity $T_s(N,p,nrhs)$ of
%\eqref{a:distributedsolve} is $\MA{O}(nrhs \times s\frac{N}{p}\log{p})$, and
%the communication complexity is $\MA{O}(nrhs \times s\log^2{p})$.

\begin{algorithm}[!htp]
\begin{algorithmic}
  \IF {$\alpha$ is at level-$\log{p}$}
    \STATE \texttt{Solve}($\bu$). %\algcmt{$\MA{O}(nrhs \times \frac{N}{p}\log{\frac{N}{p}})$}
  \ELSE
    \STATE \texttt{DistributedSolve}($c(\alpha)$, $\bu$, $\frac{q}{2}$). %\algcmt{$\MA{O}(T_s(\frac{N}{2},\frac{p}{2},nrhs))$}
    \STATE Compute $V\bu$. %\algcmt{$\MA{O}(nrhs \times s\frac{N}{p})$}
    \STATE \{0\} \texttt{Reduce} $V\bu$. %\algcmt{$\MA{O}(nrhs \times s\log{p})$}
    %\STATE \{0\} \texttt{Recv} $Vb$ from \{$\frac{p}{2}$\}. \algcmt{$\MA{O}(nrhs \times s)$}
    \STATE \{0\}  Compute $ZV\bu$ using \eqref{e:blocksmw}. %\algcmt{$\MA{O}(nrhs \times s^{2})$}
    %\STATE \{0\} \texttt{Send} $x$ to \{$\frac{p}{2}$\}.  \algcmt{$\MA{O}(nrhs \times s)$}
    \STATE \{0\} \texttt{Bcast} $ZV\bu$. %\algcmt{$\MA{O}(nrhs \times s\log{p})$}
    \STATE Compute $\bw=\bu-WZV\bu$. %\algcmt{$\MA{O}(nrhs \times s \frac{N}{p})$}
  \ENDIF
\end{algorithmic}
\caption{{} $\bw=\texttt{DistributedSolve}(\alpha, \bu, q)$}
\label{a:distributedsolve}
\end{algorithm}

{\bf Complexity.}
We use a network model to derive the parallel complexity.
For simplicity, we assume that the network topology provides 
$\MA{O}(\log{p})$ \texttt{Bcast} and \texttt{Reduce}, and
we only use the order of the 
overall message size to simplify the the communication model
without discussing the latency and the bandwidth.

Let $T^{s}(r,q)$ be the parallel complexity of the solving phase 
with $r$ right hand side and $q$ processes. The base case 
$T^{s}(r,1)=\MA{O}(rn\log{n})$ is the complexity of \algref{a:solve}.
We can derive the complexity recursively as:
\begin{equation}
  T^{s}(r,q) = T^{s}(r,\frac{q}{2}) + \MA{O}(rns+rs^2) + \MA{O}(sr\log{q}).
\end{equation}
Here $\MA{O}{(rns+rs^2)}$ is the computation cost of \eqref{e:blocksmw}, and
$\MA{O}(sr\log{q})$ is the communication cost.
The overall complexity is 
$\MA{O}(rn\log{n} + rn\log{p}) + \MA{O}(sr\log^{2}{p})$ including
both computation and communication.
Observe that the communication cost doesn't scale with the problem size
$N$, instead it's only related to $r$, $s$ and $p$.
%$\MA{O}(rn\log{n})$ is the complexity of solving the local subtree. 
%$\MA{O}(rn\log{p})$ is the distributed computation cost, $\MA{O}(rn)$
%per level. 
%$\MA{O}(r\log^{2}{p})$ is the communication complexity.
%Each level contains $\MA{O}(r\log{p})$ collective communication,
%and there are $\log{p}$ levels in total.

We derive $T^{f}(q)$ as the 
parallel complexity of the factorization phase with a fixed
skeleton size $s$ similarly. The base case 
$T^f(1) = \MA{O}(n\log^{2}{n})$ is the complexity of \algref{a:factor}.
We derive the complexity recursively as:
\begin{equation}
  T^f(q) = T^f(\frac{q}{2}) + T^s(s,\frac{q}{2}) + \MA{O}(s^3+ ns) + \MA{O}(sd+s^2).
\end{equation}
Here $T^s(s,\frac{q}{2})$ is the cost spent in \algref{a:distributedsolve}, 
$\MA{O}(s^3+ ns)$ includes the cost of \eqref{e:innerid}, and
$\MA{O}(sd+s^2)$ is the communication cost spent on broadcasting the
skeleton coordinates and the projection matrix.
Overall, the complexity is 
$\MA{O}(n\log^{2}{N})+\MA{O}(s^2\log^{3}{p}+d\log^{2}{p})$ 
including both computation and communication.
Observe that the sequential complexity is $p$ times the parallel
computation complexity, which indicates that the algorithm should
be able to achieve almost linear scalability. 
Overall the communication cost is minor, since it doesn't scale with $N$.


%$\MA{O}(n\log^{2}{n})$ is the complexity of factorizing the local subtree.
%$\MA{O}(n\log{n}\log{p}+n\log^{2}{p})$ is the distributed computation cost,
%$\MA{O}(n\log{n}+n\log{p})$ per level including the solving complexity.
%$\MA{O}(s^2\log^{3}{p}+d\log^{2}{p})$ is the communication complexity.
%Each level contains an $\MA{O}(s^2\log^{2}{p}+d\log{p})$ collective communication,
%and there are $\log{p}$ levels in total.



%{\bf Complexity:}
%The overall work doesn't change in the distributed factorization
%and solver, but the depth (the length of the critical path) can be shorten
%due to the parallelism.
%In \algref{a:distributedfactor} and \algref{a:distributedsolve},
%we traverse the distributed tree level by level. 
%Thus, the depth of the method is accumulated from each level, 
%and the depth of each level is the sum of all statement's depth.
%Each statement can either involve computation or communication.
%For the communication part, we assume that the network topology
%of the distributed system has a $\log{q}$ collective broadcasting
%and reducing.
%Thus, the local communicator \texttt{Bcast} and \texttt{Reduce}
%in level-$l$ scales $\MA{O}(\log{p}-l)$ with the message size, 
%since there are $q=2^{\log{p}-l}$ processes involved in the LC.  
%In the following, we derive the depth of our algorithms, and the
%separate the complexity into computation and communication. 

%Given that each process has $n=\frac{N}{p}$ points, we use 
%$T^f(q)$ to denote the depth
%of \algref{a:distributedfactor} with $q$ processes and $T^s(r,q)$ to 
%denote the depth of \algref{a:distributedsolve} with $r$ right hand
%sides and $q$ processes.
%Given that $T^s(r,1)=\MA{O}(rn\log{n})$, the depth is anatomized as:  
%\begin{eqnarray}
%  \label{e:solvedepth}
%  T^s(r,p) & = & T^s(r,\frac{p}{2}) + \MA{O}{(rns+rs^2)} + \MA{O}(sr\log{p}) \\
%           & = & \MA{O}(rn\log{n} + rn\log{p}) + \MA{O}(r\log^{2}{p}).
%\end{eqnarray}
%Here $\MA{O}{(rns+rs^2)}$ is the computation cost of $Vu$, $u-UVu$ and \eqref{e:smw}.
%$\MA{O}(sr\log{p})$ is communication cost of broadcasting and reducing $Vu$.
%We derive the parallelism of \algref{a:distributedsolve} as:
%\begin{equation}
%  \frac{\MA{O}(rN\log{N})}{\MA{O}(rn\log{N})+\MA{O}(r\log^{2}{p})}.
%\end{equation}
%The parallelism is affected by the amount of communication seriously,
%since the computation here is light. In the real experiment, the network
%latency and the bandwidth result in huge coefficients on the communication cost.  
 
%We can derive the depth of \algref{a:distributedfactor} with a similar analysis.
%Given that $T^f(1) = \MA{O}(n\log^{2}{n}+s^3+ns)$, we anatomize $T_f$ as:
%\begin{eqnarray}
%  \label{e:factordepth}
%  T^f(p) &=& T^f(\frac{p}{2}) + T^s(s,\frac{p}{2}) + \\ 
%         & & \MA{O}{(\kappa n + s^3+ ns)} + \MA{O}(sd+s^2) \\
%         &=& \MA{O}(n\log^{2}{n}+n\log{n}\log{p}+n\log^{2}{p}) + \\ 
%         & & \MA{O}(\log^{3}{p}+d\log{p}).
%\end{eqnarray}
%Here $T^s(s,\frac{p}{2})$ contains both the computation and communication 
%cost of solving $\tilde{U}$ with $s$ right hand sides. 
%$\MA{O}{(\kappa n + s^3+ ns)}$ involves the computation cost of
%splitting $E$, \eqref{e:innerid} and the LU factorization in \eqref{e:smw}.
%$\MA{O}(sd+s^2)$ is the communication cost of broadcasting the skeleton
%coordinates, $P$ and the reducing $VU$.
%We derive the parallelism of \algref{a:distributedfactor} as:   
%\begin{equation}
%  \frac{\MA{O}(N\log^{2}{N})}{\MA{O}(n\log^{2}{N})+\MA{O}(\log^{3}{p}+d\log{p})}.
%\end{equation}
%The computation term scales almost linear if we omit the $O(\kappa n + s^3 + ns)$
%term in \eqref{e:factordepth}, and the communication cost is minor due to 
%the $\MA{O}(n\log^{2}{N})$ computation cost.

{\bf Discussion.}
Despite that the communication cost is not a bottleneck, \IASKIT{}
shares the common problem of all treecodes: (1) the parallelism shrinks
exponentially when traversing to the root, and (2) the possible global 
synchronization during the level by level traversal. 
Solving \eqref{e:smw} in a distributed node reduces the $VW$ product
to one process in the subcommunicator. This allows us to take the 
advantage of the collective \texttt{Bcast} and \texttt{Reduce}, but
the parallelism shrinks during the solving phase.
This efficiency degradation is not significant when $p$ and $s$ are
small, but we will observe this effect in the scaling experiments.
The load-balancing problem happens when the adaptive skeletonization
strategy is used to dynamically decide the rank of $U$ and $V$.
Processes with a smaller rank will finish the factorization earlier
and wait at the global barrier until other process to finish.
This situation requires a more sophisticate schedule to prevent
the process from idling.

%\cite{march2015algebraic} has addressed the parallelism shrinking
%problem in skeletonzation, and here we address the global synchronization
%problem resulted from solving the reduced system in \eqref{e:smw}.
%To reduce communication, each process must own the correct portion of $V$ and $U$.
%This allows us to use collective communication routines in \eqref{e:smw},
%but the parallelism of a distributed node shrinks during the solving phase.
%Solving \eqref{e:smw} scales $\MA{O}(s^3)$, which is not significant when $s$
%is small. When $s$ is large, the term $s$ is no longer a constant in 
%\eqref{e:solvedepth} and \eqref{e:factordepth}.
%This situation requires a more sophisticate schedule to prevent the parallelism 
%from shrinking, and it's beyond the scope of this paper.
%Local rank 0 reduces $VU$ from all MPI processes to solve a $2s \times 2s$ inverse
%problem, and the results are broadcast back to all processes to complete
%the backward projection.
%This reduce the size of the collective communication to $\MA{O}(rs\log{p})$ 
%in each level, but the parallelism shrinks during the solving phase. 

%{\bf $U$ and $V$ distribution:}
%Since $\XX$ is distributed, starting from level $\log(p)$, constructing $U$ and $V$ 
%requires point coordinates from multiple MPI processes. 
%$U$ and $V$ involve in the distributed factorization and distributed solver,
%and their sizes are related to the problem size $N$.
%\begin{equation}
%  U^{(2)}V^{(2)} =
%  \begin{bmatrix}
%  & U_{1}^{(2)}V_{2}^{(2)} & & \\
%  U_{2}^{(2)}V_{1}^{(2)} & & & \\
%  & & & U_{3}^{(2)}V_{4}^{(2)} \\
%  & & U_{4}^{(2)}V_{3}^{(2)} & \\
%  \end{bmatrix}    
%\end{equation}
%To avoid communication becoming a performance bottleneck, in each level the left
%child must possess $U_{1}$, $V_{1}$, and the right child owns $U_{2}$, $V_{2}$. 
%the $U$  matrix must avoid any 
%communication on $U$ and $V$.
%This allows us to factorize \eqref{e:smw} by only reducing a $s \times s$ $VU$.
%Solving \eqref{e:smw}  
% with a \texttt{REDUCE} and a \texttt{BCAST}.
%With the observation in \eqref{smw}, we can find that the reduced system
%only requires $VU$ from all processors; thus, once $U$ and $V$ have been computed
%on the process  
%To compute $V$ from the children, the left child compute $V=P(:,1:s)V_{child}$,
%and the right child compute
 

%Given $N$ points in an arbitrary $d$ dimensional space, suppose we have
%$\frac{N}{m}$ hierarchical partitions such that each leaf node has no more 
%than $m$ points. This kernel matrix is called a HODLR matrix if 
%$\|K(\alpha_i,\alpha_j) - UV\| < \epsilon$. 
%Suppose that $U$, $V$ have rank no higher than $p$, then HODLR matrix can
%be factorized in $O(p^3N\log^2(N))$, and the inverse can be solved in
%$O(p^3N\log(N))$ for a single right hand side.


%{\bf Overall complexity:}
%The over all factorization complexity is
%$\MA{O}(s^{2}\frac{N}{p}(\log^{2}{p}+\log^{2}{\frac{N}{p}}))$.
%The over all solving complexity is
%$\MA{O}(s^{2}\frac{N}{p}(\log{p}+\log{\frac{N}{p}}))$.

%To modify the HODLR factorization, we relax the structure assumption 
%of $K_{12}$ and $K_{21}$, expressing the off-diagonal matrix as a
%low-rank + sparse matrix such as \eqref{e:nearfar}.
%For $K_{12}$, we replace some columns such that the remaining matrix
%can be approximated in low-rank. For $K_{21}$, this factorization 
%needs to be done on $K_{22}^{-1}K_{21}$, or the fill-in can't be controlled.
%We assume that the number of sparse columns and rows are $O(k)$.
 

%\begin{algorithm}[!htp]
%\begin{algorithmic}
%  \STATE function factor(node)
%  \IF {is leaf}
%    \STATE self interaction and lu \COMMENT{$O(m^3)$}
%  \ELSE
%    \STATE low rank + sparse factorization on $K_{12}$ \COMMENT{$O(\frac{N}{2}(p^2 + k))$}
%    \STATE factor(left child) \COMMENT{$T_f(\frac{N}{2})$}
%    \STATE factor(right child) \COMMENT{$T_f(\frac{N}{2})$}
%    \STATE solve(left child) \COMMENT{$T_s(\frac{N}{2},p)$}
%    \STATE solve(right child) \COMMENT{$T_s(\frac{N}{2},p)$}
%    \STATE solve $K_{22}^{-1}K_{21} = UV + S$ \COMMENT{$O(Np^2 + \frac{N}{2}k)$}
%    \STATE factor the sparse matrix and SMW \COMMENT{$O(Npk+Np^2)$}
%  \ENDIF
%\end{algorithmic}
%\caption{{} HODLR + Sparse Factorization, $T_f(N,p) = O(p^3N\log^2(N))$} 
%\label{a:factor2}
%\end{algorithm}
%
%\begin{algorithm}[!htp]
%\begin{algorithmic}
%  \STATE function solve(node)
%  \IF {is leaf}
%    \STATE triangular solver \COMMENT{$O(m^2(p+k)$}
%  \ELSE
%    \STATE solve(left child) \COMMENT{$T_s(\frac{N}{2},p)$}
%    \STATE solve(right child) \COMMENT{$T_s(\frac{N}{2},p)$}
%    \STATE solve the SHM problem \COMMENT{$O(Np^2 + Nk^2)$}
%  \ENDIF
%\end{algorithmic}
%\caption{{} HODLR + Sparse Solver, $T_s(N,p) = O(p(p^2+k^2)N\log(N))$} 
%\label{a:solve2}
%\end{algorithm}
%
%\begin{algorithm}[!htp]
%\begin{algorithmic}
%  \STATE function factor(node)
%  \STATE low rank + sparse factorization on $K_{12}$ \COMMENT{$O((N-m)p^2 + mk)$}
%  \STATE self interaction and lu \COMMENT{$O(m^3)$}
%  \STATE factor(rest) \COMMENT{$T_f(N-m)$}
%  \STATE solve(itself) \COMMENT{$T_s(m,p) = O(m^2(p+)$}
%  \STATE solve(rest) \COMMENT{$T_s(N-m,p)$}
%  \STATE solve $K_{22}^{-1}K_{21} = UV + S$ \COMMENT{$O((N-m)p^2 + mk)$}
%  \STATE factor the sparse matrix and SMW \COMMENT{$O(Npk+Np^2)$}
%\end{algorithmic}
%\caption{{} HODLR + Sparse Factorization, $T_f(N,p) = O(p^3N\log^2(N))$} 
%\label{a:factor3}
%\end{algorithm}
%
%\begin{algorithm}[!htp]
%\begin{algorithmic}
%  \STATE triangular solver \COMMENT{$O(m^2(p+k)$}
%  \STATE solve(rest) \COMMENT{$T_s(N-m,p)$}
%  \STATE solve the SHM problem \COMMENT{$O(Np^2 + Nk^2)$}
%\end{algorithmic}
%\caption{{} HODLR + Sparse Solver, $T_s(N,p) = O(p(p^2+k^2)N\log(N))$} 
%\label{a:solve2}
%\end{algorithm}


==> reviews.tex <==
# (1570221998): INV-ASKIT: A Parallel Fast Direct Solver for Kernel Matrices

Review #B
---------

Contribution.

In this paper the authors introduce a solver that relies on computing
efficiently an approximation of the inverse of a matrix and that can be used
for kernel matrices.

Given a matrix K, the authors propose to compute its factorization as the sum
of a diagonal matrix plus a low rank correction combined with a hierarchical
formulation. Then they compute its inverse by using the Sherman Morrison
Woodbury formula.

The factorization itself, referred to as ASKIT, was published by the last three
authors in a previous paper.  The main contribution in this paper is to focus
on the inverse, its parallel implementation, its usage for kernel matrices, and
its performance.

The paper is complete, contains the description of the algorithms, the parallel
cost (by ignoring the latency in the communication cost) and impressive
performance results on 4,096 Sandy-Bridge cores.  The authors also discuss the
accuracy of the algorithms for kernel matrices by looking at different test
cases, for example when it is used as a preconditioner for GMRES, or when it is
used in kernel regression for binary classification.  Due to probably space
limits, sometimes it is hard to understand the errors presented by the authors.
For someone not an expert in machine learning algorithms, but an expert in
scientific computing, it is not easy to see in which algorithm GMRES is needed
for example.  A better introduction of algorithms that could use the proposed
inversion algorithm would have been useful.

Suggestions for Improvement.

The paper is very nicely written, and my main comment is the one above, it
would be useful to give more details on how GMRES is used, what is the expected
accuracy, etc.

Complexity, page 7: a better notation is required in equations (15) and (16),
for example gamma-beta notation to be able to distinguish between the number
of flops (gamma term) and the volume of communication (beta term). Also, you
explain that latency costs are ignoring, but you assume that the cost of
Reduce and Bcast is O(log P).  Those seem to be latency costs for Reduce and
Bcast, the number of messages exchanged in a broadcast.  This requires some
clarification, and including the latency cost would be useful as well, since
for small messages, it dominates the cost.

Page 5, GETRF routine from LAPACK. You explain that the factorization uses LU
with column pivoting, but GETRF uses partial pivoting and I do not see how
you obtain column pivoting, if you need to use this for a low rank
approximation. Clarify.

Begining of Page 8:  It is hard to understand some of the errors, in
particular when you use \tilde{K} as a preconditioner for GMRES, some other
errors are relevant. What is the matrix that is preconditioned ? Why the
error used in the paper is relevant ?


Review #C
---------

Contribution.

This paper presents an algorithm for computing an approximate factorization of
NxN Kernel matrices. The parallel algorithm is based on an earlier paper by the
authors. In the earlier paper, a kernel matrix is approximated as a
block-diagonal-plus-low-rank matrix. In this current paper, this formulation is
used in the well-known Sherman-Morrison-Woodbury formula to invert the Kernel
matrices. The approximation from the earlier paper also allows the use of the
proposed inversion scheme as a preconditioner. Parallel algorithms are
discussed (with their limitations too) and experiments are presented.

It would be great if the authors can give experimental comparison with an
alternative. If there is no alternative to Inv-Askit, the authors could
possibly give Inv-Askit's time along with Askit.
However, if there are alternatives (what about other low rank matrix solvers),
then a comparison is needed.

Can we also have run time analysis with small numbers of cores? 

The motivation need some work. Where the inversion of kernel matrices is
required? There are many applications in which kernel matrices arise (this is
    clearly stated) but what is the use of their inversion?

* the style of the paper is not right. Probably this will take 10 pages of
with IPDPS style, but not sure.

* There are too many footnotes. Better avoid them.

* Missing references for "the idea of exploiting the block-diagonal-plus-low-rank".

* "We use \alpha and \beta to denote two siblings in the binary tree." could
be in the table as well.

* "We partition the points using geometric information and a binary tree so
that we have m points per leaf. " At this point the reader does not know if
"m" is given or computed.

* X(\alpha) in "X(\alpha)\in \alpha" is not defined.

* "We use a parallel ball tree data structure. " The "ball tree" is not known.

* Please re write the following statement "Another ASKIT algorithm for the
Separated(i,\alpha), i is separated from \alpha if \alpha does not contain
any nearest-neighbors of i. "

* In Algorithm II.1, "LU factor Z in (11)". There is no "Z" in (11).

* "For simplicity, we assume that m and s are all constant related to the
problem size N." Since "m" and "s" depend on the problem size, they cannot be
hidden in the asymptotic notation, much like the authors do not ignore them
in the asymptotic result for the storage requirements.

* The footnote 6 is rather vague. 

* Refer to Algorithm II.4 on page 6, at the right column, in the paragraph "Solver".

* "O(log p) Bcast and Reduce, " just below Algorithm II.4. 

* References are missing for SUSY and COVTYPE.

* "For example, for the MNIST dataset we the classification is whether a point is digit 3 or not."


Review #D
---------

Contribution.

The authors introduce their toolkit INV-ASKIT for factorization of
high-dimensional kernel matrices. The authors present parallel algorithms
targeting shared and distributed memory architectures and empirical results on
two platforms. They build on their earlier work and extend it significantly. It
is a well-written paper that provides sufficient background and features a
strong experimental section.

The authors present a theoretical analysis of the complexity of the proposed
algorithm. Since this paper represents their recent work, it has several
limitations. Several of these limitations have been documented in the paper.
The methods are well described, and the previous work, ASKIT, has been
summarized in manner that provides sufficient background. The paper has a good
description of the parallel algorithm, supporting data structures, and
complexity analysis. 

Similar to other treecodes, INV-ASKIT also has several limitations in a
parallel context such as loss of parallel efficiency during tree traversal and
synchronization between levels. Consequently, these limitations are observed in
scaling experiments. 

Experiments are conducted on two parallel platforms with differing features,
and four datasets from different application domains such as
high-energy physics, cartography, standard machine learning, and
handwritten digit recognition. The authors perform strong and weak
scaling.  Gaussian kernel with values chosen from cross-validation
is used for experiments. The authors conduct 29 experiments between
strong and weak scaling and kernel regression for the four datasets
on the two platforms.

Scaling results are quickly summarized in three tables. The runtime
is dominated by the factorization time. Time for communication and
solving are not dominant. Factorization time is separated as local
and distributed, where the distributed time dominates in most
cases. Although communication cost is negligible, the loss of
parallel efficiency is attributed to the lower concurrent work
during the computation of approximate inverse using the
Sherman-Morrison-Woodbury (SMW) formula. Machine utilization varies
for different datasets from eight per cent to 45 per cent.  The
authors attribute this variance in scalability among datasets to
issues arising from load balancing, especially from nodes with
larger values of s that become bottleneck in the critical path
(arising from adaptive skeletonization). The authors provide
excellent weak scaling results. 

In summary, scaling up to 4096 cores are provided for new parallel
factorization algorithm of high dimensional kernel matrices,
demonstrating up to 50 per cent utilization of peak floating point
operation performance of hardware.

Suggestions for Improvement.

The presentation of experimental results, especially the scaling results, can
be greatly improved. One has to struggle through the current presentation to
understand different aspects.


Review #E
---------

Contribution.

The authors present a parallel scheme for applying the inverse of a shifted
high-dimensional kernel matrix and provide thorough performance experiments for
certain classes of matrices.

While the work is certainly impressive, there is a large amount of
misinformation that would suggest that the work is more original than it
actually is. For example, there is an explicit claim that the only previous
parallel work is by Wang et al., when, in fact, numerous authors have worked in
the area over the past decade (with Kriemann et al. suggesting both the
	earliest and most diverse family of techniques). Closely related to this
issue is the complete lack of discussion of low-rank approximation schemes
which require sufficient separation between the source and target domains
(which some of the authors are certainly aware of due to their work on FMM) and
their importance for low-rank approximations in multiple dimensions, even for
the Laplace equation (despite the authors' suggestion that Helmholtz is
	required for their suggested scheme to have super-constant rank growth).
Factoring structured matrices with more general admissibility conditions is
known to be a significantly harder problem and so Newton-Schulz schemes tend to
be preferred in said context.

Thus, the authors have made qualitatively incorrect implications about the
asymptotic complexity of their scheme and made bold and incorrect claims about
previous work. For example, parallel domain decomposition schemes (in the lingo
	of Kriemann et al.) have been ignored, as have Newton-Schulz schemes, which
are the best-known technique for non-trivial admissibility properties.

While these issues are certain to be vexing to experts in the area, the core
algorithmic contributions and discussion are of use and so I would recommend
the paper as a weak accept and hope that the authors exercise more care in the
future.


